iCPS-DL: A Description Language for Autonomic Industrial Cyber-Physical Systems

Modern industrial systems require frequent updates to their cyber and physical infrastructures, often demanding considerable reconfiguration effort. This paper introduces the industrial Cyber-Physical Systems Description Language, iCPS-DL, which enables autonomic reconfigurations for industrial Cyber-Physical Systems. The iCPS-DL maps an industrial process using semantics for physical and cyber-physical components, a state estimation model, and agent interactions. A novel aspect is using communication semantics to ensure live interaction among distributed agents. Reasoning on the semantic description facilitates the configuration of the industrial process control loop. A Water Distribution Networks domain case study demonstrates iCPS-DL's application.

==> figures/fig_composing_IIoT_control.tex <==
\begin{figure*}
\[
\begin{array}{c}
    \begin{array}{c}
        \rolemap; \set{\p[i]: \tinact \setbar i \in I} \proves \ginact \has \set{\p[i]: \tinact \setbar i \in I}
        \\[1mm]
        \rolemap; \set{\p[i]: \tvar{t} \setbar i \in I} \proves \var{t} \has \set{\p[i]: \tvar{t} \setbar i \in I}
    \end{array}
    \qquad
    \tree {
        \rolemap; \LLd, \p: \locald[1], \q: \locald[2] \proves \glob \has \LL, \p: \local[1], \q: \local[2]
    }{
        \rolemap; \LLd, \p: \intro{\q}{\locald[2]} \locald[1] \proves \conn{\p}{\q} \glob \has \LL, \p: \intro{\q}{\local[2]} \local[1]
    }
    \\[5mm]
    \tree {
        \rolemap; \set{\p[i]: \tvar{t} \setbar i \in I}, \set{\p[j]: \locald[j] \setbar j \in J} \proves \glob \has \set{\p[i]: \tvar{t} \setbar i \in I}, \set{\p[j]: \local[j] \setbar j \in J}
        \qquad
        \forall j \in J, \local[j] \not= \tvar{t}
    }{
        \rolemap; \set{\p[i]: \tinact \setbar i \in I}, \set{\p[j]: \trec{t} \locald[j] \setbar j \in J} \proves \rec{t} \glob \has \set{\p[i]: \tinact \setbar i \in I}, \set{\p[j]: \trec{t} \local[j] \setbar j \in J}
    }
    \\[5mm]
    \tree{
        \forall \in I,\ \rolemap; \LLd, \p: \local[{i_1}], \q: \local[{i_2}] \proves \globd[i] \has \LL, \p: \local[i], \q: \locald[i]
        \qquad \rolemap[\p, {\rr[1]}] = \q
        \qquad \rolemap[\q, {\rr[2]}] = \p
        %\\%[0mm]
        %[\rolemap[\p, \rr_1] = \rolemap[\q, \rr_2] = v_s] \lor (\rolemap[\p, \rr_1] = \undef, \rolemap[\p, \rr_2] = \undef, \rr[1] = \q, \rr[2] = \p)
    }{
        \rolemap; \LLd, \p: \Tor{i \in I} \out{\rr[1]}{\U[i]} \local[{i_1}], \q: \Tor{i \in I} \inp{\rr[2]}{\U[i]} \locald[{i_2}] \proves \Gor{i \in I} \pass{\p}{\q}{\U[i]} \glob[i] \has \LL, \p: \Tor{i \in I} \out{\q}{\U[i]} \local[i], \q: \Tor{i \in I} \inp{\p}{\U[i]} \locald[i]
    }
\end{array}
\]
    \caption{The protocol composition with participant renaming relation \label{fig:iiot_composition}}
\end{figure*}

==> figures/fig_composition_example.tex <==


\begin{figure}
    \[
    \arraycolsep=2pt
    \begin{array}{rcl|}
        &&  \multicolumn{1}{l}{\lrangle{\rAG, \modelmap}}
        \\[1mm]
        \cline{3-3} &&
        \\[-2mm]
        \localhead &=&
            \trec{t} \out{\consumerp}{\headt} \tvar{t},
            \quad
            \localflow = \trec{t} \out{\consumerp}{\flowt} \tvar{t}
        \\
        \localest &=&
             \inp{\supervisor}{\init} \trec{t} \inp{\producerp[1]}{\flowt} \inp{\producerp[2]}{\flowt} \out{\consumerp}{\headt} \tvar{t}
        \\
        \localcontrol &=&
            \trec{t} \inp{\producerp}{\headt} (\out{\pumpp}{\ON} \tvar{t} \tor \out{\pumpp}{\OFF} \tvar{t})
        \\
        \localsuperv &=&
            \intro{\estp}{\localest} \nout{\estp}{\init}
            \quad
            \localpump = \trec{t} (\inp{\controller}{\ON} \tvar{t} \tor \inp{\controller}{\OFF} \tvar{t})
        \\[2mm]
        \rAG &=& \rAG[s] \cup \rAG[g] \cup \rAG[c]
        \\
        &&\rAG[s]
              =     \levelSensor:       \localhead,
                    \flowSensor:        \localflow
        \qquad \quad
        \rAG[g]
            =       \estp:              \localest
        \\ 
        &&\rAG[c]
              =     \controller:        \localcontrol, 
                    \supervisor:        \localsuperv,
                    \pumpp:             \localpump
        \\[2mm]
        \modelmap &=& \set{\flowSensor \maparrow \Sensors[f], \levelSensor \maparrow \Sensors[h], \estp \maparrow \eVg[m]}
        \\[1mm]
        \hline
        %\hline
        \\[-1mm]
        &&  \multicolumn{1}{l}{\rolemap_1; \LL[1] \proves \globsimple[1] \has \LLsimple[1]}
        \\[1mm]
        \cline{3-3} &&
        \\[-2mm]
        \LL[1]
            &=& \levelSensor:           \localflow,
                \pumpp:                 \localpump,
                \controller:            \localcontrol
        \\[2mm]
        \contextmap_1
            &   \multicolumn{1}{l}{:}& \treesimple[1] \to \LL[1]
        \\
        \contextmap_1
            &=& \set{s_6 \maparrow \levelSensor,\ \tank.\head \maparrow \controller}
        \\
        \rolemap_1
            &=& \set{
                    (\levelSensor, \consumerp) \maparrow \controller,
                    (\controller, \producerp) \maparrow \levelSensor,
                    (\controller, \pumpp) \maparrow \pumpp,
            \\  &&  (\pumpp, \controller) \maparrow \controller
                }
        \\[2mm]
        \LLsimple[1]
            &=& \levelSensor:          \trec{t} \out{\controller}{\headt} \tvar{t}, \ 
                                        \pumpp: \trec{t} (\inp{\controller}{\ON} \tvar{t} \tor \inp{\controller}{\OFF} \tvar{t})
        \\  &&  \controller:           \trec{t} \inp{\levelSensor}{\headt} (\out{\pumpp}{\ON} \tvar{t} \tor \out{\pumpp}{\OFF} \tvar{t}),
        \\[1mm]
        \globsimple[1]
            &=& %\multicolumn{2}{l}{
                    \rec{t} \pass{\levelSensor}{\controller}{\headt} (\pass{\controller}{\pumpp}{\ON} \var{t} \gor \pass{\controller}{\pumpp}{\OFF} \var{t})
        \\[1mm]
        \hline
        \\[-1mm]
        &&  \multicolumn{1}{l}{\rolemap_2; \LL[2] \proves \globsimple[2] \has \LLsimple[2]}
        \\[1mm]
        \cline{3-3}  &&
        \\[-2mm]
        \LL[2]  &=&     \flowSensor[1]:  \localflow, \flowSensor[2]: \localflow,
                        \supervisor: \localsuperv, \pumpp: \localpump,
                        \controller: \localcontrol
        \\[2mm]
        \contextmap_2
            &   \multicolumn{1}{l}{:}& \treesimple[2] \to \LL[2]
        \\
        \contextmap_2 &=&
                        \set{
                            s_5 \maparrow \flowSensor[1],
                            s_6 \maparrow \flowSensor[2],
                            \tank.\mass \maparrow \estp
                        }
        \\
        \rolemap_2    &=&
                        \set{
                            (\flowSensor[1], \consumerp) \maparrow \estp,
                            (\flowSensor[2], \consumerp) \maparrow \estp,
                            (\estp, \producerp[1]) \maparrow \flowSensor[1],
        \\            & &   (\estp, \producerp[2]) \maparrow \flowSensor[2],
                            (\estp, \consumerp) \maparrow \controller
                            (\controller, \producerp) \maparrow \estp,
        \\            & &   (\controller, \pumpp) \maparrow \pumpp,
                            (\pumpp, \controller) \maparrow \controller
                        }
        \\[2mm]
        \hline
    \end{array}
    \]
    \caption{Control loop protocol for the \WDNsimple Water Distribution Network\label{fig:composition_example}}
\end{figure}
